Not All Fabrics Are Created Equal: Exploring eFPGA Parameters For IP Redaction

Semiconductor design houses rely on third-party foundries to manufacture their integrated circuits (IC). While this trend allows them to tackle fabrication costs, it introduces security concerns as external (and potentially malicious) parties can access critical parts of the designs and steal or modify the Intellectual Property (IP). Embedded FPGA (eFPGA) redaction is a promising technique to protect critical IPs of an ASIC by \textit{redacting} (i.e., removing) critical parts and mapping them onto a custom reconfigurable fabric. Only trusted parties will receive the correct bitstream to restore the redacted functionality. While previous studies imply that using an eFPGA is a sufficient condition to provide security against IP threats like reverse-engineering, whether this truly holds for all eFPGA architectures is unclear, thus motivating the study in this paper. We examine the security of eFPGA fabrics generated by varying different FPGA design parameters. We characterize the power, performance, and area (PPA) characteristics and evaluate each fabric's resistance to SAT-based bitstream recovery. Our results encourage designers to work with custom eFPGA fabrics rather than off-the-shelf commercial FPGAs and reveals that only considering a redaction fabric's bitstream size is inadequate for gauging security.

==> x_discusison.tex <==
% \section{Discussion\label{sec:discussion}}
% \todoblock{Add things like parts of the eFPGA design that we did not explore in these experiments, such as fracturable LUT?}
% This study has presented some of the key concepts that one has to take care of while approaching redaction based logic obfuscation. We have shown our study focussing on only two FPGA parameters \textit{K} and \textit{N} from the \autoref{tab:arch_param}. There are still so many decision left to a designer to select from a varieties of parameters. This study will serve as building a road to encourage more to dive into the FPGA architecture, and look into how one can make a more efficient fabric that will gives best result in terms of PPA and Security.
% The study is done on more conventional LUTs, but one can also do similar study for modern day's \textit{fracturable LUTs}, which is shown to a more efficient compared to the previous LUTs, as now we can map more than one function within a LUTs, with just addition of few gates to accommodate logic to separate two different outputs of a LUTs. This will put some level of efforts in the routing (local and global), where now one has to accommodate a more numbers of input and outputs, but the cost of this enhancement will have slight change in the overhead compared to mapping two different function in separate LUTs in a conventional FPGA design, this will increase the resource utilization as shown in ~\cite{LUT,FPGA_arch, fpga_ref}, which is one of the factor that a designer should consider(\autoref{sec:practical}). \newline
% For our study we have keep parameters: \textit{W},  \textit{$F_{c,in}$}, \textit{$F_{c,out}$}, \textit{$F_s$} and \textit{$L$}, fixed depending on the previous study's on FPGA to give best results in terms of PPA. The impact of varying this parameters and evaluate their security will enhance the future study on (PPA-S). For instance, we can have more than one eFPGA in our SoCs, where one has routing channel width \textit{W} of 40 and other has \textit{W} as 100, this will surely impact the PPA numbers, as there are more routing to be done with increase in the routing tracks, this will eventually change the \textit{$F_{c,in}$} and \textit{$F_{c,out}$}  values thus forcing both \textit{local routing and global routing} to maximise effort. From the perspective of attack, for partially unrolled IcySAT attack experiment, we  limited number of unroll factors to 3 (10, 20 and 30) due to time constraints. However, to have more precise information on the exact unroll factor at which bit-stream could be recovered, an attack series with integral sweep on unroll factor has to be done. Moreover, for designs where all 3 unroll factors failed to recover the correct bit-stream, higher unroll factors with higher time-outs may recover the correct keys. For instance, the partially unrolled IcySAT could successfully recover the keys for K4N3 variant of 4x4 eFPGA fabric for an unroll factor of 40. Hence wider sweep of unroll factor is required to evaluate the security of fabrics better.   
% \begin{itemize}
%     \item Other threat models: 
% \end{itemize}




==> x_dse.tex <==
\section{Design Space Exploration\label{sec:results}}
\subsection{Experimental Setup}

%The security of redaction techniques  directly relates to the security strength of the FPGA fabric \cite{chen_decoy_2020}.%, rest of the functionality of the design implemented with regular ASIC flow is known to all. 
In this section we have shown the result of the impact of different FPGA architectures on Area, Power, Delay and security. We conduct a thorough study by tuning the parameters \autoref{sec:fpga_arch} in an architecture file using~\cite{XTang_tvlsi_2018}. The overhead increases with the complexity of the architecture. We varied the number of inputs of a  LUT (k) from 3-7 and the  number of clusters (N) from 2-8 so as to be efficient in terms of PPA overhead. The study explores the security strength of each fabric with these different configurations for k and N. This way, we  deduce what combination of FPGA fabric parameters  make it SAT-attack hard. 

One can develop a theoretical claims based on the FPGA parameters. However, the FPGA structures used in the industry are complex and building a mathematical model of fabrics is out of scope of this study. Instead, we conduct an empirical analysis to study SAT-attack resiliency by sweeping the parameters. This will guide us in selecting fabrics that are efficient in terms of PPA and  security. An increase in the bitstream results in non-linear distribution among the bits used for routing, configuring LUTs and I/Os. we have come up with the hypothesis that not each of the part of the bitstream contributes equally in the security of the fabric, routing have more impact compared to configuration bitstream as it increases the complexity of SAT solver.

%To maintain consistency between the redaction technique and the threat model, we assume that we have the netlist post-layout. 

The area, delay and power calculations use the data taken after  synthesis, placement and floorplan  generated through OpenFPGA flow~\cite{XTang_tvlsi_2018}. This flow is highlighted in \autoref{fig:redact-flow}. For synthesis we use Cadence GENUS 18.14 and for layout implementation we use Cadence INNOVUS 18.10. For floorplanning we set the utilization to 70\% to have a faster timing closure. %Since, the purpose of the study is to show the trends when we one move from one configuration parameter to another rather than an optimised implementation. 
We use FreePDK 45~nm technology library~\cite{FreePDK45} for our study. 

\subsubsection{Area}
\autoref{tab:area_result} shows the distribution of area for different FPGA architecture. The analysis is straight forward with increase in N value across k, the complexity of the CLB, routing increases due to more number of inputs and output coming in and out of a tile \autoref{sec:fpga_arch}. A bigger design can be accommodated with increase in N values for a particular k. Our study guides a designer with area values continuously increase from the smallest change one can achieve when moving from one fabric to another.  For a particular N values with increase in k values, similar trend is achieved,since now the inputs to the LUTs increases which overall increase the input to CLBs, as calculated from the formula for I~\cite{LUT}. With increase in the inputs and outputs, the connection block and switch block \autoref{sec:fpga_arch} complexity also increase which eventually increases the routing components, thus more area is needed for a fabric. A designer can select a fabric size and configuration with the available area budget that can be spent on redaction and the security guarantee as shown in \autoref{sec:security}. Although the study point to with more area comes more security as is clear from \autoref{sec:security}, one has to be aware of the overall increase in area when the eFPGA is combined with the rest of design \autoref{fig:redact-flow}. This is not a simple addition of the two areas as the tools need to do optimisations as the surrounding logic changes. So by selecting a larger fabric, one pays a huge penalty in terms of overhead. 
%%%%%%%%%%%% %   4x4      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[b!]
% \centering
% \caption{Area ($\mu m^2$) 4x4 Fabric}
% \label{tab:area_4x4}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &6019.58	&6595.47&	8223.66	&11209.42&	15621.91 \\\hline
%  3 &7422.46	&8096.77&	11057.62&	15580.95&	22942.77\\\hline
				
%  4& 8787.31	&10961.86	&15672.19&	24487.35&	30558.08\\\hline
				
% 5&10338.89&	13879.08&	17883.18&	29477.06&	39926.60\\\hline
				
% 6&12881.32&	16006.28&	22458.91&	31695.23&	46417.53\\\hline
				
% 7&14470.40&	18613.35&	26128.91&38366.24&	58477.17\\\hline
				
% 8&16767.58&	22774.65&	30682.57&	47307.31&	67507.61\\\hline

 
%  \end{tabular}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 5x5      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{table}[b!]
% \centering
% \caption{Area ($\mu m^2$) 5x5 Fabric}
% \label{tab:area_5x5}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &12381.50&	15745.87&	19274.89&	25188.61&	36952.18 \\\hline
%  3 &15006.92 & 18382.19	&	25567.12&	33448.17&	53361.46\\\hline
				
%  4& 18418.90&	24469.07&35259.36 &	48989.22&	68923.53\\\hline
				
% 5&24748.11	&32640.33	&39748.91&	68745.57&	84538.79\\\hline
				
% 6&26873.18&	35187.01&	51709.34&	76729.22	&107220.88\\\hline
				
% 7&33930.69&	43431.15&	59311.08&	87152.24&	133015.16\\\hline
				
% 8&39201.22&	50143.39&	67747.54&	103520.28&	155193.44 \\\hline

 
%  \end{tabular}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         6x6                               %%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b!]
% \centering
% \caption{Area ($\mu m^2$) 6x6 Fabric}
% \label{tab:area_6x6}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &20447.69&	27885.58&	33623.19&	51125.20&	69842.82 \\\hline
%  3 &25034.32&	31953.25&	47343.48&	65900.44&	96467.29\\\hline
				
%  4& 36032.36&	45500.90&	68472.12&	87479.42&	127315.58\\\hline
				
% 5&41904.04&	56004.71&	67310.24&	121652.17&	159183.44\\\hline
				
% 6&52687.95	&64872.88	&86037.43&	127583.71&	183012.52\\\hline
				
% 7&57587.14&	73238.02&	101013.50&	150442.95&219576.62	\\\hline
				
% 8&67155.42&	85809.74&	116823.48& 155791.94&224047.81  \\\hline

 
%  \end{tabular}
% \end{table}
\begin{table*}[t]
%\begin{threeparttable}
\centering
\caption{Area for different eFPGA fabrics for different configuration parameters.}
\label{tab:area_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
& \multicolumn{15}{c}{Area ($mm^2$)} \\ \cmidrule{2-16}
& \multicolumn{5}{c|}{4x4} & \multicolumn{5}{c|}{5x5} & \multicolumn{5}{c}{6x6} \\ \cmidrule{1-6} \cmidrule{7-11} \cmidrule{12-16}
 \backslashbox[2cm]{K}{N} & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } \\
& & & & & & & & & & & & & & & \\ \midrule
2 & 0.006	&0.007	&0.008&	0.011&	0.016& 0.012	&0.016	&0.019	&0.025	&0.037 &0.020&	0.028&	0.034&	0.051&	0.070\\ \midrule
3 & 0.007&	0.008&	0.011&	0.016&	0.023 &0.015	&0.018	&0.026	&0.033	&0.053 &0.025&	0.032&	0.047&	0.066&	0.096\\\midrule
4 & 0.009&	0.011&	0.016&	0.024&	0.031 &0.018	&0.024	&0.035	&0.049	&0.069 &0.036&	0.046&	0.068&	0.087&	0.127 \\ \midrule
5 & 0.010&	0.014&	0.018&	0.029&	0.040 &0.025	&0.033	&0.040	&0.069	&0.085 &0.042&	0.056&	0.067&	0.122&	0.159\\ \midrule
6 & 0.013&	0.016&	0.022&	0.032&	0.046 &0.027	&0.035	&0.052	&0.077	&0.107  &0.053&	0.065&	0.086&	0.128&	0.183 \\ \midrule
7 & 0.014&	0.019&	0.026&	0.038&	0.058 &0.034	&0.043	&0.059	&0.087	&0.133 & 0.058&	0.073&	0.101&	0.150&	0.220\\ \midrule
8 & 0.017&	0.023&	0.031&	0.047&	0.068 &0.039	&0.050	&0.068	&0.104	&0.155 & 0.067&	0.086&	0.117&	0.156&	0.224\\ \bottomrule
\end{tabular} } 
\end{table*}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Delay}

Compared to our study on area, the delay presents some interesting results \autoref{tab:delay_result}. As it was also mentioned in~\cite{LUT, FPGA_arch} the changes in delay is not a linear function of K and N, some architecture have better delay number as compared to other and is independent of complexity of the design. As can be seen from our results, for a particular N delay values improves as one goes from a low k value to high reaching best result for the maximum k(=7), there is a slight change in trend for some N, where k=6 \autoref{tab:area_4x4} gives the optimal solution, \autoref{tab:area_6x6}, but one can generalise as there are only few cases of such changes. The study on delay is important where performance of the device is really important. We have tried to give a overview on delay in \autoref{sec:proposed}, where if a design to redact selected is in critical path, and with the integration of fabric with rest of ASIC, it will put a huge load on the tools to meet the timing specification and even may be not able to meet. In that case selecting a fabric with the least(or best) delay by looking at a different combination of K and N is of utmost priority.    


\begin{table*}[t]
%\begin{threeparttable}
\centering
\caption{Delays for different eFPGA fabrics with different configuration parameters.}
\label{tab:delay_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
& \multicolumn{15}{c}{Delay (ns)} \\ \cmidrule{2-16}
& \multicolumn{5}{c|}{4x4} & \multicolumn{5}{c|}{5x5} & \multicolumn{5}{c}{6x6} \\ \cmidrule{1-6} \cmidrule{7-11} \cmidrule{12-16}
 \backslashbox[2cm]{K}{N} & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } \\
& & & & & & & & & & & & & & & \\ \midrule
2 & 1.85 & 1.96 & 1.91 & 1.22 & 1.68 & 3.74 & 2.82 & 2.24 & 2.24 & 1.67 & 6.47 & 4.41 & 3.74 & 3.84 & 4.46 \\ \midrule
3 & 1.86 & 1.52 & 1.91 & 1.39 & 1.10 & 3.15 & 2.37 & 3.63 & 3.58 & 2.64 & 5.64 & 3.78 & 5.91 & 3.81 & 4.11 \\\midrule
4 & 1.88 & 1.29 & 1.41 & 1.28 & 1.56 & 3.99 & 3.21 & 3.15 & 3.59 & 2.48 & 6.93 & 5.24 & 5.07 & 4.23 & 3.61 \\ \midrule
5 & 1.77 & 2.06 & 1.65 & 1.77 & 1.35 & 5.34 & 3.45 & 4.14 & 3.36 & 3.37 & 8.92 & 6.21 & 4.89 & 6.19 & 3.74 \\ \midrule
6 & 2.58 & 1.67 & 1.65 & 1.88 & 1.41 & 5.30 & 3.39 & 3.93 & 3.21 & 2.52 & 8.72 & 6.21 & 4.86 & 5.28 & 3.51 \\ \midrule
7 & 2.55 & 2.43 & 1.83 & 1.59 & 1.23 & 6.43 & 4.83 & 3.99 & 3.21 & 2.58 & 8.73 & 5.89 & 4.74 & 5.22 & 3.65 \\ \midrule
8 & 2.43 & 2.12 & 1.77 & 1.82 & 1.83 & 6.52 & 4.71 & 3.72 & 3.06 & 2.81 & 8.74 & 5.94 & 4.54 & 5.02 & 3.33 \\ \bottomrule
\end{tabular} } 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 4x4         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b!]
% \centering
% \caption{Delay (ns) 4x4 Fabric}
% \label{tab:delay_4x4}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &1.85&	1.96&	1.91	&1.22&	1.68 \\\hline
%  3 &1.86&	1.52&	1.91&	1.39&	1.10\\\hline
				
%  4& 1.88&	1.29&	1.41&	1.28&	1.56\\\hline
				
% 5&1.77&	2.06&	1.65&	1.77&	1.35\\\hline
				
% 6&2.58&	1.67&	1.65&	1.88&	1.41\\\hline
				
% 7&2.55&	2.43&	1.83&	1.59&	1.23\\\hline
				
% 8&2.43&	2.12&	1.77&	1.82&	1.83\\\hline

 
%  \end{tabular}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   5x5        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b!]
% \centering
% \caption{Delay (ns) 5x5 Fabric}
% \label{tab:delay_5x5}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &3.74&	2.82&	2.24&	2.24	&1.67 \\\hline
%  3 &3.15&	2.37&	3.63&	3.58&	2.64\\\hline
				
%  4&3.99&	3.21&	3.15&	3.59&	2.48\\\hline
				
% 5&5.34&	3.45	&4.14	&3.36&	3.37\\\hline
				
% 6&5.30&	3.39&	3.93&	3.21&	2.52\\\hline
				
% 7&6.43&	4.83&	3.99&	3.21&	2.58\\\hline
				
% 8&6.52&	4.71&	3.72	&3.06&	2.81\\\hline

 
%  \end{tabular}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  6x6 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[b!]
% \centering
% \caption{Delay (ns) 6x6 Fabric}
% \label{tab:delay_6x6}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &6.47&	4.41&	3.74&	3.84&	4.46 \\\hline
%  3 &5.64&	3.78&	5.91&	3.81&	4.11\\\hline
				
%  4&6.93	&5.24&	5.07&	4.23&	3.61\\\hline
				
% 5&8.92&	6.21	&4.89	&6.19	&3.74\\\hline
				
% 6&8.72&	6.21	&4.86	&5.28&	3.51\\\hline
				
% 7&8.73&	5.89&	4.74&	5.22&3.65	\\\hline
				
% 8&8.74&	5.94&	4.54&	5.02&3.33	\\\hline

 
%  \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Security Analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Power}
The study on power is shown in \autoref{tab:power_result}. Similar to study on area, we have seen that power increases with increase in complexity of the fabric (k and N). For a particular value of N, with increase in k values there is a increasing trend followed and vice versa. If one look at the two extreme end, one being smallest architecture of (k=3 and N=2) and the other with (k=7 and N=8), there is almost a 10x increase in power for a same 4x4 fabric, this trend is also followed with all other fabric sizes of 5x5 and 6x6. This shows the complexity of the fabric with just increasing k and N values, now there are more switches and more routing is required to map a design, which eventually increases bitstream sizes, and makes the fabric more SAT resilient shown in \autoref{sec:security}. The power will constraint one to go for a larger fabric if the application involved either battery driven or edge devices where one employs low power devices. The result shows the trend that power follows and one can always come up with a more power compact architecture, which is beyond the scope of this paper. We want to show the general trend that is being followed across different fabrics rather than the most optimised design possible. 



\begin{table*}[t]
%\begin{threeparttable}
\centering
\caption{Power for different eFPGA fabrics for different configuration parameters.}
\label{tab:power_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
& \multicolumn{15}{c}{Power (mW)} \\ \cmidrule{2-16}
& \multicolumn{5}{c}{4x4} & \multicolumn{5}{c}{5x5} & \multicolumn{5}{c}{6x6} \\ \cmidrule(l){2-6} \cmidrule(l){7-11} \cmidrule(l){12-16}
 \backslashbox[2cm]{N}{K} & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } \\
& & & & & & & & & & & & & & & \\ \midrule
2 & 0.71 & 0.79 & 0.98 & 1.31 & 1.94 & 1.56 & 2.06 & 2.45 & 3.19 & 4.85 & 2.62 & 3.75 & 4.45 & 6.76 & 9.24 \\\midrule
3 & 0.89 & 0.98 & 1.39 & 1.92 & 2.84 & 1.88 & 2.36 & 3.33 & 4.25 & 6.98 & 3.22 & 4.18 & 6.44 & 8.64 & 13.06 \\ \midrule
4 & 1.07 & 1.39 & 1.99 & 2.63 & 3.87 & 2.33 & 3.34 & 4.68 & 6.35 & 9.14 & 4.84 & 6.34 & 9.31 & 11.63 & 17.23 \\ \midrule
5 & 1.31 & 1.77 & 2.35 & 3.75 & 5.03 & 3.30 & 4.52 & 5.46 & 9.35 & 11.16 & 5.74 & 7.92 & 9.48 & 16.57 & 21.44 \\ \midrule
6 & 1.62 & 2.09 & 3.02 & 4.02 & 5.58 & 3.53 & 4.86 & 7.44 & 10.35 & 13.68 & 7.36 & 9.44 & 12.61 & 17.56 & 23.13 \\ \midrule
7 & 1.92 & 2.51 & 3.58 & 4.86 & 7.14 & 4.89 & 6.19 & 8.69 & 11.41 & 16.12 & 8.46 & 10.80 & 15.12 & 20.63 & 28.31 \\ \midrule
8 & 2.20 & 3.07 & 4.28 & 5.97 & 8.17 & 5.65 & 7.33 & 10.21 & 14.14 & 19.52 & 9.73 & 12.98 & 17.95 & 21.44 & 30.43 \\ \bottomrule
\end{tabular}}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 4x4         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b!]
% \centering
% \caption{Power (mW) 4x4 Fabric}
% \label{tab:power_4x4}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 & 0.71	&0.79&	0.98&	1.31&	1.94\\\hline
%  3 &0.89&	0.98&	1.39&	1.92&	2.84\\\hline
				
%  4& 1.07&	1.39&	1.99&	2.63&	3.87\\\hline
				
% 5&1.31&	1.77&	2.35&	3.75&	5.03\\\hline
				
% 6&1.62&	2.09&	3.02	&4.02	&5.58\\\hline
				
% 7&1.92&	2.51&	3.58&	4.86&	7.14\\\hline
				
% 8&2.20&	3.07&	4.28&	5.97&	8.17\\\hline

 
%  \end{tabular}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   5x5        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b!]
% \centering
% \caption{Power (mW) 5x5 Fabric}
% \label{tab:power_5x5}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 & 1.56&	2.06&	2.45&	3.19&	4.85\\\hline
%  3 &1.88	&2.36&	3.33&	4.25&	6.98\\\hline
				
%  4&2.33	&3.34	&4.68	&6.35&	9.14\\\hline
				
% 5&3.30	&4.52&	5.46&	9.35&	11.16\\\hline
				
% 6&3.53	&4.86&	7.44&	10.35&	13.68\\\hline
				
% 7&4.89&	6.19&	8.69&	11.41&	16.12\\\hline
				
% 8&5.65&	7.33&	10.21&	14.14&	19.52\\\hline

 
%  \end{tabular}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  6x6 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[b!]
% \centering
% \caption{Power (mW) 6x6 Fabric}
% \label{tab:power_6x6}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &2.62&	3.75&	4.45&	6.76&	9.24 \\\hline
%  3 &3.22&	4.18&	6.44&	8.64&	13.06\\\hline
				
%  4&4.84	&6.34&	9.31&	11.63&	17.23\\\hline
				
% 5&5.74	&7.92&	9.48&	16.57	&21.44\\\hline
				
% 6&7.36	&9.44&	12.61&	17.56&	23.13\\\hline
				
% 7&8.46	&10.80&	15.12&	20.63&	28.31\\\hline
				
% 8&9.73&	12.98&	17.95	&21.44	&30.43\\\hline

 
%  \end{tabular}
% \end{table}

\begin{table*}[t]
%\begin{threeparttable}
\centering
\caption{Bitstream size for different eFPGA fabrics for different configuration parameters.}
\label{tab:bitstream_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
& \multicolumn{15}{c}{Bitstream} \\ \cmidrule{2-16}
& \multicolumn{5}{c}{4x4} & \multicolumn{5}{c}{5x5} & \multicolumn{5}{c}{6x6} \\ \cmidrule{2-6} \cmidrule{7-11} \cmidrule{12-16}
\backslashbox[2cm]{N}{K} & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } & \multirow{2}{*}{ 3 } & \multirow{2}{*}{ 4 } & \multirow{2}{*}{ 5 } & \multirow{2}{*}{ 6 } & \multirow{2}{*}{ 7 } \\
& & & & & & & & & & & & & & & \\
2 & 642 & 680 & 856 & 1166 & 1712 & 1265 & 1553 & 1958 & 2684 & 3893 & 2090 & 2739 & 3322 & 5037 & 7313 \\
3 & 766 & 851 & 1107 & 1559 & 2475 & 1539 & 1908 & 2493 & 3501 & 5725 & 2574 & 3309 & 4430 & 6635 & 10326 \\
4 & 878 & 1090 & 1518 & 2019 & 3262 & 1786 & 2370 & 3344 & 4974 & 7150 & 3533 & 4392 & 6137 & 8598 & 13144 \\
5 & 982 & 1357 & 1782 & 2775 & 3958 & 2354 & 3161 & 3926 & 6748 & 8710 & 3935 & 5369 & 6786 & 11510 & 15525 \\
6 & 1195 & 1509 & 2053 & 2969 & 4661 & 2429 & 3302 & 4780 & 6948 & 10693 & 4679 & 6059 & 8251 & 11947 & 18348 \\
7 & 1284 & 1688 & 2312 & 3388 & 5552 & 3030 & 3948 & 5379 & 7598 & 12714 & 5134 & 6766 & 9310 & 13770 & 21660 \\
8 & 1434 & 1890 & 2614 & 4030 & 6361 & 3321 & 4356 & 6007 & 9211 & 14378 & 5647 & 7487 & 10420 & 16116 & 25305 \\ \bottomrule
\end{tabular}}
\end{table*}












% \begin{table}[b!]
% \centering
% \caption{Bitstream of 4x4 Fabric}
% \label{tab:bit_4x4}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 &642&	680&	856	&1166&	1712 \\\hline
%  3 &766&	851&	1107&	1559&	2475\\\hline
				
%  4&878	&1090	&1518	&2019	&3262\\\hline
				
% 5&982&	1357&	1782&	2775&	3958\\\hline
				
% 6&1195	&1509	&2053	&2969	&4661\\\hline
				
% 7&1284&	1688&	2312&	3388&	5552\\\hline
				
% 8&1434	&1890&	2614	&4030&	6361\\\hline

 
%  \end{tabular}
% \end{table}



% \begin{table}[b!]
% \centering
% \caption{Bitstream of 5x5 Fabric}
% \label{tab:bit_5x5}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 & 1265	&1553	&1958&	2684&	3893\\\hline
%  3 &1539&	1908&	2493&	3501&	5725\\\hline
				
%  4&1786&	2370&	3344&	4974&	7150\\\hline
				
% 5&2354	&3161&	3926&	6748&	8710\\\hline
				
% 6&2429&	3302&	4780&	6948&	10693\\\hline
				
% 7&3030	&3948&	5379	&7598&	12714\\\hline
				
% 8&3321&	4356&	6007&	9211&	14378\\\hline

 
%  \end{tabular}
% \end{table}


% \begin{table}[b!]
% \centering
% \caption{Bitstream of 6x6 Fabric}
% \label{tab:bit_6x6}
% \begin{tabular}{|c|c|c|c|c|c|} \hline

%  \backslashbox[1cm]{N}{K}
%  & 3 &4 &5&6&7\\\hline
%  2 & 2090&	2739&	3322&	5037&	7313\\\hline
%  3 &2574&	3309&	4430&	6635&	10326\\\hline
				
%  4&3533&	4392&	6137&	8598&	13144\\\hline
				
% 5&3935&	5369&	6786&	11510	&15525\\\hline
				
% 6&4679&	6059&	8251	&11947	&18348\\\hline
				
% 7&5134&	6766&	9310&	13770&	21660\\\hline
				
% 8&5647&	7487&10420	&16116&	25305\\\hline

 
%  \end{tabular}
% \end{table}

